Inferring Type II-P Supernova Progenitor Masses from Plateau Luminosities

Connecting observations of core-collapse supernova explosions to the properties of their massive star progenitors is a long-sought, and challenging, goal of supernova science. Recently, Barker et al. (2022) presented bolometric light curves for a landscape of progenitors from spherically symmetric neutrino-driven core-collapse supernova (CCSN) simulations using an effective model. They find a tight relationship between the plateau luminosity of the Type II-P CCSN light curve and the terminal iron core mass of the progenitor. Remarkably, this allows us to constrain progenitor properties with photometry alone. We analyze a large observational sample of Type II-P CCSN light curves and estimate a distribution of iron core masses using the relationship of Barker et al 2022. The inferred distribution matches extremely well with the distribution of iron core masses from stellar evolutionary models, and namely, contains high-mass iron cores that suggest contributions from very massive progenitors in the observational data. We use this distribution of iron core masses to infer minimum and maximum mass of progenitors in the observational data. Using Bayesian inference methods to locate optimal initial mass function parameters, we find M$_{\mathrm{min}}=9.8^{+0.37}_{-0.27}$ and M$_{\mathrm{max}}=24.0^{+3.9}_{-1.9}$ solar masses for the observational data.

==> journal_abbr.tex <==
\newcommand\aj{AJ}% 
          % Astronomical Journal 
\newcommand\araa{ARA\&A}% 
          % Annual Review of Astron and Astrophys 
\newcommand\apj{ApJ}% 
          % Astrophysical Journal 
\newcommand\apjl{ApJ}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}% 
          % Astrophysical Journal, Supplement 
\newcommand\ao{Appl.~Opt.}% 
          % Applied Optics 
\newcommand\apss{Ap\&SS}% 
          % Astrophysics and Space Science 
\newcommand\aap{A\&A}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{A\&A~Rev.}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{AZh}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}% 
          % Bulletin of the AAS 
\newcommand\jrasc{JRASC}% 
          % Journal of the RAS of Canada 
\newcommand\memras{MmRAS}% 
          % Memoirs of the RAS 
\newcommand\mnras{MNRAS}% 
          % Monthly Notices of the RAS 
\newcommand\pra{Phys.~Rev.~A}% 
          % Physical Review A: General Physics 
\newcommand\prb{Phys.~Rev.~B}% 
          % Physical Review B: Solid State 
\newcommand\prc{Phys.~Rev.~C}% 
          % Physical Review C 
\newcommand\prd{Phys.~Rev.~D}% 
          % Physical Review D 
\newcommand\pre{Phys.~Rev.~E}% 
          % Physical Review E 
\newcommand\prl{Phys.~Rev.~Lett.}% 
          % Physical Review Letters 
\newcommand\pasp{PASP}% 
          % Publications of the ASP 
\newcommand\pasj{PASJ}% 
          % Publications of the ASJ 
\newcommand\qjras{QJRAS}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{S\&T}% 
          % Sky and Telescope 
\newcommand\solphys{Sol.~Phys.}% 
          % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% 
          % Soviet Astronomy 
\newcommand\ssr{Space~Sci.~Rev.}% 
          % Space Science Reviews 
\newcommand\zap{ZAp}% 
          % Zeitschrift fuer Astrophysik 
\newcommand\nat{Nature}% 
          % Nature 
\newcommand\iaucirc{IAU~Circ.}% 
          % IAU Cirulars 
\newcommand\aplett{Astrophys.~Lett.}% 
          % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{Fund.~Cosmic~Phys.}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{Geochim.~Cosmochim.~Acta}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}% 
          % Geophysics Research Letters 
\newcommand\jcp{J.~Chem.~Phys.}% 
          % Journal of Chemical Physics 
\newcommand\jgr{J.~Geophys.~Res.}% 
          % Journal of Geophysics Research 
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{Nucl.~Phys.~A}% 
          % Nuclear Physics A 
\newcommand\physrep{Phys.~Rep.}% 
          % Physics Reports 
\newcommand\physscr{Phys.~Scr}% 
          % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}% 
          % Planetary Space Science 
\newcommand\procspie{Proc.~SPIE}% 
          % Proceedings of the SPIE 
\newcommand\jcphys{J.~Comp.~Phys.}% 
          % Journal of Computational Physics

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

